Model and Feature Diversity for Bayesian Neural Networks in Mutual Learning

Bayesian Neural Networks (BNNs) offer probability distributions for model parameters, enabling uncertainty quantification in predictions. However, they often underperform compared to deterministic neural networks. Utilizing mutual learning can effectively enhance the performance of peer BNNs. In this paper, we propose a novel approach to improve BNNs performance through deep mutual learning. The proposed approaches aim to increase diversity in both network parameter distributions and feature distributions, promoting peer networks to acquire distinct features that capture different characteristics of the input, which enhances the effectiveness of mutual learning. Experimental results demonstrate significant improvements in the classification accuracy, negative log-likelihood, and expected calibration error when compared to traditional mutual learning for BNNs.

==> table/table_tmp.tex <==
\begin{table}
  \caption{Comparison of classification accuracy on CIFAR-100 dataset when only partial data are retained based on the uncertainties of the predictions.}
  \label{tab:cifar100}
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{lc|cc|cc|cc}

    \hline
    \multicolumn{2}{c|}{Network Types}  & \multicolumn{2}{c|}{vanilla} & \multicolumn{2}{c|}{DML} & \multicolumn{2}{c}{Ours} \\
    
    Net1 & Net2 & Net1 & Net2 &Net1 & Net2 & Net1 & Net2  \\
    \hline 
    ResNet20* & ResNet20 & 89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02 &89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02  \\
                           
    \hline
  \end{tabular}}
\end{table}

\begin{table}
  \caption{Comparison of classification accuracy on CIFAR-100 dataset when only partial data are retained based on the uncertainties of the predictions.}
  \label{tab:cifar100}
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{l|c|cccc}

    \hline
     Method & Model & Lowest accuracy & Highest Accuracy &  Ensembled Accuracy \\
    \hline 
    \multirow{2}{*}{Vanila} & ResNet20 &  &  &      \\
                            &  ResNet20* &  &  &      \\
    \cdashline{1-6}
        \multirow{2}{*}{DML} & ResNet20 &  &  &     \\
                            &  ResNet20* &  &  &     \\
    \cdashline{1-6}
        \multirow{2}{*}{Ours} & ResNet20 &  &  &     \\
                            &  ResNet20 *&  &  &     \\
    \hline
  \end{tabular}}
\end{table}


\begin{table}
  \caption{Classification score on CIFAR10 dataset}
  \label{tab:cifar100}
  \centering
  \resizebox{0.7\columnwidth}{!}{
  \begin{tabular}{l|ccc}

    \toprule
     % & \multicolumn{3}{c|}{Vanila} & \multicolumn{3}{c|}{DML} & \multicolumn{3}{c}{Ours}\tabularnewline
      & Vanilla & DML & Ours \\
     % & ACC $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & ACC $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & ACC $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$\tabularnewline
    \hline 
    \hline 
    ResNet8 &  &  &   \\
    ResNet8* &  &  &    \tabularnewline
    ResNet20 & 89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02 & 89.55 $\pm$ 0.02  \\
    ResNet20* &  &  &    \tabularnewline
  %  \cdashline{1-4}
    ResNet56 &  &  &   \tabularnewline
    ResNet56* &  &  &   \tabularnewline
   % \cdashline{1-4}
    WRN-16-2 &  &  & \tabularnewline
    WRN-16-2* &  &  &   \tabularnewline
    \bottomrule
  \end{tabular}}
\end{table}


\begin{table}
%   \caption{Classification score on CIFAR100 dataset}
%   \label{tab:ci}
%   \centering
%  % \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{l|ccc|cc}

%     \hline
%      % & \multicolumn{3}{c|}{Individual} & \multicolumn{3}{c|}{DML} & \multicolumn{3}{c}{Ours}\tabularnewline
     
%      & DNN  & MC-Dropout  & MFVI  & DML & Ours   \tabularnewline
%     \hline 
%     \hline 

%     ResNet20 & \multirow{2}{*}{69.06}  & \multirow{2}{*}{70.13} & 63.18 $\pm$ 0.2 & 67.27 $\pm$ 0.2 & 68.32 $\pm$ 0.2  \\
%     ResNet20* &  &  & 67.62 $\pm$ 0.2  & 69.61 $\pm$ 0.2 &  70.45 $\pm$ 0.2\tabularnewline
%     \cdashline{1-6}
%     WRN-16-2 &  &  &  &  &  \tabularnewline
%     WRN-16-2 &  &  &  &  &  \tabularnewline

%     \hline
%   \end{tabular}
% \end{table}


\begin{table}
  \caption{Classification score on CIFAR10 dataset}
  \label{tab:ci}
  \centering
 % \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{l|ccc|cc}

    \hline
     % & \multicolumn{3}{c|}{Individual} & \multicolumn{3}{c|}{DML} & \multicolumn{3}{c}{Ours}\tabularnewline
     
     & DNN  & MC-Dropout  & MFVI  & DML & Ours   \tabularnewline
    \hline 
    \hline 

    ResNet20 & 89.93 $\pm$ 0.2 & 89.93 $\pm$ 0.2 & 89.93 $\pm$ 0.2 & 89.93 $\pm$ 0.2 & 89.93 $\pm$ 0.2  \\
    ResNet20* & 92.47 & - & - & 92.67 &  \tabularnewline
    \cdashline{1-6}
    WRN-16-2 &  &  &  &  &  \tabularnewline
    WRN-16-2 &  &  &  &  &  \tabularnewline

    \hline
  \end{tabular}
\end{table}

==> tex/background.tex <==
\section{Background}
\paragraph{Bayesian neural networks} provide a probabilistic interpretation of deep neural networks by representing distributions over the weight parameters $w$. Given training dataset $\mathcal{S}=\{x, y\}$ with input $x = \{x_i\}_{i=1}^N$ and corresponding output $y = \{y_i\}_{i=1}^N$. In the Bayesian setting, we want to learn an approximate posterior distribution $q(w; \theta)$ to maximize the likelihood distribution $p(\calS|w) = p(y|f(x; w))$. This can be obtained by minimizing the KL divergence between the approximate posterior distribution $q(w; \theta)$ and the true posterior $p(w|S)$:

\begin{equation}
    \begin{split}
    \theta^* & = \argminA_\theta \mathrm{KL}[ q(w; \theta) \Vert p(w|\calS)] \\
            & = \argminA_\theta \mathrm{KL}[ q(w; \theta) \Vert p(w)] - \int_{\Theta} q(w; \theta) \log p(y|x,w) \dd w \\
            & = \argminA_\theta \mathrm{KL}[ q(w; \theta) \Vert p(w)] + \mathbb{E}_{q(w; \theta)} \left[ - \sum_{n=1}^N \log p(y_n|x_n, w) \right],
    \end{split}
\end{equation}
where \(p(w)\) is the prior of the parameter \(w\) and \(\theta\) is the paramter space.
%\cnguyen{where \(p(w)\) is the prior of the parameter \(w\) and \(\Theta\) is the paramter space.}

\emph{Bayes by Backprop} (BBB) \cite{blundell2015weight} is a simple but efficient variational approach. They suppose the approximate posterior following a Gaussian distribution with a diagonal covariance matrix, i.e., \(q(w; \theta) = \mathcal{N}(\mu, \mathrm{diag}(\sigma^{2}))\) and apply a parametrization trick to represent each weight in the neural network by a mean and a standard deviation:

\begin{equation}
    w = \mu + \sigma \odot \epsilon, \quad \epsilon \sim \mathcal{N}(0, I),
\end{equation}
where: \(\odot\) is the Hadamard product and \(I\) is the identity matrix.

However, the standard BBB method in practice is sensitive to hyperparameters. To address this issue, in \cite{farquhar_radial_2020}, the authors introduce a variant of BBB called Radial Bayesian Neural Network, where weight parameters are sampled as follows:
\begin{equation}
    w = \mu + \sigma \odot \frac{\epsilon}{\norm{\epsilon}} r, \quad r = \abs{\rho} \quad  \textnormal{for} \quad \rho \sim \mathcal{N}(0, I),
\end{equation}
where \(\norm{.}\) denotes the vector norm.

==> tex/method_save.tex <==
\section{Proposed method}
\label{sec:proposed}

\subsection{Overview of Bayesian Neural Networks}


% Bayesian posterior
% \begin{equation}
%     p(\theta|D) = \frac{p(D|\theta)p(\theta)}{\int p(D|\theta)p(\theta)d\theta}
% \end{equation}

% In the inference, bayesian model averaging (BMA)
% \begin{equation}
%     p(y^*|D) = E_{p(\theta|D)}[p(y|x, \theta)] = \int p(y|x, \theta) p(\theta|D) d\theta 
% \end{equation}
Bayesian neural networks provide a probabilistic interpretation of deep neural networks by representing distributions over the weight parameters $w$. Given training dataset $\mathcal{S}=\{X, Y\}$ with input $X = \{x_i\}_{i=1}^N$ and corresponding output $Y = \{y_i\}_{i=1}^N$. In the Bayesian setting, we want to learn an approximate posterior distribution $q(w; \theta)$ to maximize the likelihood distribution $p(\calS|w) = p(y|f(x; w))$. This can be obtained by minimizing the KL divergence between the approximate posterior distribution $q(w; \theta)$ and the true posterior $p(w|S)$ using KL divergence.

% \begin{equation}
%     \begin{split}
%     KL[ q_\phi(\theta) || p(\theta|S)]
%             & =  KL[ q_\phi(\theta) || p(\theta)] - \int q_\phi(\theta) \log p(y|\theta)d\theta + const\\
%             & =  KL[ q_\phi(\theta) || p(\theta)] - \mathbb{E}_{q_\phi(\theta)}[\sum_{n=1}^N \log p(y_n|x_n, \theta)] + const
%     \end{split}
% \end{equation}

% \begin{equation}
%     L(\phi) = \argminA_\phi KL[ q_\phi(\theta) || p(\theta|D)]
% \end{equation}

% \begin{equation}
%     \begin{split}
%     \phi^* & = \argminA_\phi KL[ q_\phi(\theta) || p(\theta|D)] \\
%             & = \argminA_\phi KL[ q_\phi(\theta) || p(\theta)] - \int q_\phi(\theta) \log p(y|\theta)d\theta \\
%             & = \argminA_\phi KL[ q_\phi(\theta) || p(\theta)] - \mathbb{E}_{q_\phi(\theta)}[\sum_{n=1}^N \log p(y_n|x_n, \theta)]
%     \end{split}
% \end{equation}

\begin{equation}
    \begin{split}
    \theta^* & = \argminA_\theta KL[ q(w; \theta) || p(w|\calS)] \\
            & = \argminA_\theta KL[ q(w; \theta) || p(w)] - \int q(w; \theta) \log p(y|x,w)dw \\
            & = \argminA_\theta KL[ q(w; \theta) || p(w)] + \mathbb{E}_{q(w; \theta)}[- \sum_{n=1}^N \log p(y_n|x_n, w)]
    \end{split}
\end{equation}

We adopt Bayes by Backprop (BBB) \cite{blundell2015weight} method which is a simple but efficient variational approach. They suppose the approximate posterior $q(w; \theta)$ following a Gaussian distribution with a diagonal variation and apply a parametrization trick to represent each weight in the neural network by a mean and a standard deviation. 

\begin{equation}
    w = \mu + \sigma \odot \epsilon, \quad \epsilon \sim \mathcal{N}(0,I)
\end{equation}
However, the standard BBB method in practice is sensitive to hyperparameters. In our work, we adopt a variant of BBB called Radial Bayesian Neural Network \cite{farquhar_radial_2020}, with a small modification when sampling weight parameters as follows:
\begin{equation}
    w = \mu + \sigma \odot \frac{\epsilon}{||\epsilon||}r, \quad r = |\rho| \quad  \textnormal{for} \quad \rho \sim \mathcal{N}(0,I)
\end{equation}

\subsection{Deep Mutual Learning for Bayesian Neural Networks}

We formulate our proposed method by considering two peer Bayesian networks, $S1$ and $S2$, with the goal of constructing an efficient framework for Bayesian Deep Mutual Learning. Specifically, we aim to enhance diversity by
%in mutual learning not only in logits but also in the feature space. Additionally, we 
leveraging the benefits of Bayesian neural networks over deterministic neural networks, in which weights in BNNs are represented by a distribution. In other words, we increase the distance of posterior distributions and subsequently enhance the diversity in Bayesian mutual learning. By doing so, the peer Bayesian networks can learn more meaningful representations. To the best of our knowledge, this is the first work that exploits the model parameter space to enhance diversity in mutual learning. To further enhance diversity, we also exploit the diversity in feature space.



%To make the BNN models generalize better and converge in different modes, we  
\subsection{Diversity in model parameter space}
In our setting, the approximate posterior distributions for peer Bayesian models are Gaussian distributions with diagonal covariance matrices:
\begin{equation}
    \begin{cases}
      q(w; \theta) = \mathcal{N}[w|\mu_\theta, \Sigma_\theta = \text{diag}(\sigma_\theta^2)]\\
      q(w; \phi) = \mathcal{N}[w|\mu_\phi, \Sigma_\phi = \text{diag}(\sigma_\phi^2)], 
    \end{cases}       
\end{equation}

where $\mu_\theta, \sigma_\theta, \mu_\phi, \sigma_\phi \in \mathbb{R}^d$, with d denoting the number of model parameters. 

To measure the distance between two posterior distributions, We investigate two widely used methods to measure the distance between two posterior distributions including KL diversion and optimal transport.


\begin{equation}
    L_{\text{param}} = D(q(w;\theta) || q(w; \phi))
\end{equation}

-present advantage of OT over KL
- The optimal transport between two Gaussians
\begin{equation}
    \mathcal{W}_2^2(q(w; \theta), q(w; \phi)) = ||\mu_\theta - \mu_\phi||^2 + \mathcal{B}(\Sigma_\theta, \Sigma_\phi)^2
\end{equation}
Where Bures distance is represented by:
\begin{equation}
    \begin{split}
    \mathcal{B}(\Sigma_\theta, \Sigma_\phi)^2 
    & = tr(\Sigma_\theta + \Sigma_\phi - 2(\Sigma_\theta^{1/2} \Sigma_\phi \Sigma_\theta^{1/2})^{1/2}) \\
    & = ||\theta - \phi||^2_2
    \end{split}
\end{equation}





To promote diversity in the parameter space, we propose minimizing the following loss function instead of directly maximizing $L_{\text{param}}$:

\begin{equation}
    L_{\text{diverse param}} = \text{log}(1 + exp(- D(q(w;\theta) || q(w; \phi)))
\end{equation}

The above loss function exhibits desirable properties: $L \ge 0$, and minimizing L implies maximizing $D(q(w;\theta) || q(w; \phi))$, thereby enhancing diversity in the model parameter space. These properties make optimization more stable during training. 


\subsection{Diversity in feature space}

We aim to leverage intermediate features to increase the distance between the distribution of features among peer networks, rather than directly matching features using L2 distance in offline distillation methods such as FitNets \cite{FitNets} and Attention transfer \cite{AT}. This is because directly matching features can lead to peer networks becoming identical, thereby reducing diversity in mutual learning. The backbone networks are divided into the same blocks according to their depth. Let $F^{S1}_k$ and $F^{S2}_k$ be extracted features at block $k^{th}$ of Bayesian models, $S1$ and $S2$, respectively. Let $\mathcal{I}$ be the selected layer indices for intermediate features.
In our approach, we aim to increase the diversity of feature distributions among peer Bayesian models by maximizing their distance from each other. 
However, directly maximizing the distance between $F^{S1}_k$ and $F^{S2}_k$ may be sensitive to parameter updates and harmful during the mutual learning process. To address this, we propose combining features from different blocks of each Bayesian network using cross-attention ~\cite{SA}. This allows for enhanced capacity and the ability for each block to have its own parameters and updates, promoting diversity during the training process. Specifically, given extracted features from the block $k^{th}$, and block $(k+1)^{th}$ of network $S1$, the combined feature using cross-attention is expressed as:
\begin{equation}
    F'^{S1} = u({F^{S1}_k}, {F^{S1}_{k+1}}) = \text{softmax}((\bW_QF^{S1}_{k+1})(\bW_KF^{S1}_k)^T)\bW_VF^{S1}_k,
\end{equation}
where $\bW_Q$, $\bW_K$, and $\bW_V$ represent learnable parameters for query, key, and value, respectively. Similary, we have combined features $F'^{S2}=u({F^{S2}_k}, {F^{S2}_{k+1}})$. 
The distance between fused feature distributions of peer Bayesian networks are computed as $D_{feat}(F'^{S1}, F'^{S2})$, 
% \begin{equation}
%     L_{feat} = D_{feat}(F'^{S1}, F'^{S2})
% \end{equation}
where D is the loss measuring distances between probability distributions in the feature space, different forms of D can be applied in our proposed method. Similar to the measurement of distance in the parameter space, we utilize KL divergence and Optimal Transport. In offline knowledge distillation, \cite{PKT} and \cite{WoCRD} apply KL divergence and Wasserstein distance, respectively, to transfer the probability distribution from teacher to student instead of their actual representation. However, due to the fact that the distribution of the feature space may not be clearly represented by a Gaussian distribution, and other forms of optimal transport are often computationally extensive, we adopt KL divergence simmilar in \cite{PKT} as a measurement of distance. Given the $\mathcal{P}$ and $\mathcal{Q}$ is the probability distribution of features from Bayesian model $S1$ and $S2$, respectively
\begin{equation}
    D_{KL}(F'^{S1}, F'^{S2}) = D_{KL}(\mathcal{P} || \mathcal{Q}) = \int \mathcal{P}(x) \frac{\mathcal{P}(x) }{\mathcal{Q}(x)}dx
\end{equation}
Similar to diversity in parameter space, we also propose minimizing the following loss function instead of directly maximizing $D_{KL}(F'^{S1}, F'^{S2})$:

\begin{equation}
    L_{\text{diverse feat}} = \text{log}(1 + exp(- D_{KL}(F'^{S1}, F'^{S2})))
\end{equation}

% where D is the loss measuring distances between probability distributions in feature space. Different forms of D can be applied in our proposed method. Simmilar the measurement of the distance in parameter space, we utilize the KL divergence and Optimal transport. In offline knowlege distillation, In \cite{PKT} and \cite{WoCRD}, they apply KL divergence and Wasserstein disance to transfer the probability distribution from teacher to student, instead of their actual representation, respectively. However, due to the distribution of feature space could not clearly represent by Gaussian distribution, and other form of optimal transport often computational extensive, therefore, we adopt the KL divergence as a measurement distance. 
%Given the $\mathcal{P}$ and $\mathcal{Q}$ is the probability distribution of features from Bayesian model $S1$ and $S2$, respectively:

% \begin{equation}
%     \calL_{feat} = \calD(u({F^{S1}_k1}_{k=1}))
% \end{equation}






